VerifyThis 2019: A Program Verification Competition (Extended Report)

VerifyThis is a series of program verification competitions that emphasize the human aspect: participants tackle the verification of detailed behavioral properties -- something that lies beyond the capabilities of fully automatic verification, and requires instead human expertise to suitably encode programs, specifications, and invariants. This paper describes the 8th edition of VerifyThis, which took place at ETAPS 2019 in Prague. Thirteen teams entered the competition, which consisted of three verification challenges and spanned two days of work. The report analyzes how the participating teams fared on these challenges, reflects on what makes a verification challenge more or less suitable for the typical VerifyThis participants, and outlines the difficulties of comparing the work of teams using wildly different verification approaches in a competition focused on the human aspect.

==> tab_problems-classification.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-2 package
% Sun Aug  4 17:07:21 2019
\begin{table*}[ht]
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{llrrlllllrr}
  \toprule
{\textsc{problem}} & {\textsc{competition}} & {\textsc{order}} & {\textsc{time}} & {\textsc{sequential}} & {\textsc{input}} & {\textsc{output}} & {\textsc{algorithm}} & {\textsc{mutable}} & {\textsc{partial}} & {\textsc{complete}} \\ 
  \midrule
Maximum by elimination & VT11 & 1 & 60 & sequential & array & simple & iterative & immutable & 83 & 67 \\ 
  Tree maximum & VT11 & 2 & 90 & sequential & tree & simple & outlined & immutable & 100 & 17 \\ 
  Find duplets in array & VT11 & 3 & 90 & sequential & array & simple & find & immutable & 83 & 50 \\ 
  Longest common prefix & VT12 & 1 & 45 & sequential & array & simple & iterative & immutable & 100 & 73 \\ 
  Prefix sum & VT12 & 2 & 90 & sequential & array & complex & outlined & immutable & 73 & 9 \\ 
  Delete min node in binary search tree & VT12 & 3 & 90 & sequential & tree & same & recursive & mutable & 18 & 0 \\ 
  Relaxed prefix & VT15 & 1 & 60 & sequential & array & same & iterative & immutable & 79 & 7 \\ 
  Parallel GCD by subtraction & VT15 & 2 & 60 & concurrent & scalar & same & iterative & mutable & 79 & 14 \\ 
  Doubly linked lists & VT15 & 3 & 90 & sequential & linked list & same & outlined & mutable & 71 & 7 \\ 
  Matrix multiplication & VT16 & 1 & 90 & sequential & matrix & same & iterative & immutable & 86 & 43 \\ 
  Binary tree traversal & VT16 & 2 & 90 & sequential & tree & simple & iterative & mutable & 79 & 7 \\ 
  Static tree barriers & VT16 & 3 & 90 & concurrent & tree & simple & iterative & mutable & 79 & 7 \\ 
  Pair insertion sort & VT17 & 1 & 90 & sequential & array & same & iterative & mutable & 100 & 10 \\ 
  Odd-even transposition sort & VT17 & 3 & 90 & concurrent & array & same & iterative & mutable & 60 & 0 \\ 
  Tree buffer & VT17 & 4 & 90 & sequential & tree & same & recursive & immutable & 40 & 20 \\ 
  Gap buffer & VT18 & 1 & 60 & sequential & array & same & iterative & mutable & 91 & 36 \\ 
  Count colored tiles & VT18 & 2 & 90 & sequential & array & same & recursive & immutable & 55 & 18 \\ 
  Array-based queue lock & VT18 & 3 & 90 & concurrent & array & simple & iterative & mutable & 27 & 9 \\ 
  Monotonic segments and GCG sort & VT19 & 1 & 90 & sequential & array & same & iterative & immutable & 85 & 15 \\ 
  Cartesian trees & VT19 & 2 & 90 & sequential & array & complex & iterative & immutable & 69 & 15 \\ 
  Sparse matrix multiplication & VT19 & 3 & 90 & concurrent & matrix & same & iterative & immutable & 85 & 0 \\ 
   \bottomrule
\end{tabular}
\caption{For each challenge \textsc{problem} used at VerifyThis: the \textsc{competition} when it was used; the \textsc{order} in which it appeared; how much \textsc{time} (in minutes) was given to participants to solve it; whether the main algorithm is \textsc{sequential} or concurrent; the main \textsc{input} data type; whether the \textsc{output} data type is of the \textit{same} kind as the input, \textit{simple}r, or more \textit{complex}; when the \textsc{algorithm} was given in pseudo-code, whether it was \textit{iterative} or \textit{recursive} (if it was not given, whether it was \textit{outlined} or participants had to \textit{find} it based on the requirements); whether the input is \textsc{mutable} or immutable; and the percentages of participating teams that were able to submit a \text{partial} or \textsc{complete} solution.} 
\label{tab:problems-classification}
\end{table*}


==> tools_history.tex <==
\begin{tabular}{l *{7}{r} |r}
 & \multicolumn{7}{c}{\textsc{VerifyThis competition}} \\
\cmidrule(lr){2-8}
 & \multicolumn{1}{c}{2011} & \multicolumn{1}{c}{2012} & \multicolumn{1}{c}{2015} & \multicolumn{1}{c}{2016} & \multicolumn{1}{c}{2017} & \multicolumn{1}{c}{2018} & \multicolumn{1}{c}{2019} & \multicolumn{1}{c}{\textsc{by tool}} \\
\midrule
AProVe & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\
AutoProof & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 1 \\
CBMC & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 1 \\
CIVL & 0 & 0 & 0 & 1 & 1 & 1 & 0 & 3 \\
Coq & 0 & 0 & 0 & 0 & 0 & 1 & 2 & 3 \\
Dafny & 1 & 2 & 3 & 5 & 1 & 1 & 0 & 13 \\
ESC/Java2 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 1 \\
F* & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 1 \\
Frama-C & 0 & 0 & 1 & 0 & 1 & 1 & 2 & 5 \\
GNATProve & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 1 \\
Isabelle & 0 & 0 & 0 & 0 & 0 & 1 & 2 & 3 \\
jStar & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\
KeY & 1 & 1 & 1 & 1 & 2 & 1 & 0 & 7 \\
KIV & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 7 \\
mCRL2 & 0 & 0 & 1 & 1 & 0 & 0 & 1 & 3 \\
MoCHi & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 1 \\
OpenJML & 0 & 0 & 0 & 0 & 0 & 0 & 1 & 1 \\
PAT & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 1 \\
VCC & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 1 \\
VerCors & 0 & 0 & 1 & 1 & 1 & 2 & 2 & 7 \\
VeriFast & 0 & 1 & 1 & 1 & 0 & 1 & 0 & 4 \\
Viper & 0 & 0 & 0 & 1 & 0 & 1 & 1 & 3 \\
Why3 & 1 & 2 & 1 & 2 & 3 & 1 & 1 & 11 \\
\midrule
\multicolumn{1}{c}{\textsc{by competition}} & 6 & 9 & 12 & 9 & 7 & 11 & 9
\end{tabular}

